EyeNeRF: A Hybrid Representation for Photorealistic Synthesis, Animation and Relighting of Human Eyes

A unique challenge in creating high-quality animatable and relightable 3D avatars of people is modeling human eyes. The challenge of synthesizing eyes is multifold as it requires 1) appropriate representations for the various components of the eye and the periocular region for coherent viewpoint synthesis, capable of representing diffuse, refractive and highly reflective surfaces, 2) disentangling skin and eye appearance from environmental illumination such that it may be rendered under novel lighting conditions, and 3) capturing eyeball motion and the deformation of the surrounding skin to enable re-gazing. These challenges have traditionally necessitated the use of expensive and cumbersome capture setups to obtain high-quality results, and even then, modeling of the eye region holistically has remained elusive. We present a novel geometry and appearance representation that enables high-fidelity capture and photorealistic animation, view synthesis and relighting of the eye region using only a sparse set of lights and cameras. Our hybrid representation combines an explicit parametric surface model for the eyeball with implicit deformable volumetric representations for the periocular region and the interior of the eye. This novel hybrid model has been designed to address the various parts of that challenging facial area - the explicit eyeball surface allows modeling refraction and high-frequency specular reflection at the cornea, whereas the implicit representation is well suited to model lower-frequency skin reflection via spherical harmonics and can represent non-surface structures such as hair or diffuse volumetric bodies, both of which are a challenge for explicit surface models. We show that for high-resolution close-ups of the eye, our model can synthesize high-fidelity animated gaze from novel views under unseen illumination conditions.

==> 3-overview.tex <==
% -*- compile-command: "texify --pdf --quiet main.tex" -*-
% !TEX root = main.tex
% !TeX spellcheck = en_US
% (shell-command "start main.pdf")

\section{Overview}
\label{sec:overview}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth,page=1,trim={0 6.5cm 0 0},clip]{figures/architecture.pdf}
    \caption{\oursname Overview.}
    \label{fig:overview}
\end{figure*}

An overview of our proposed network is shown in Fig.~\ref{fig:overview}.
Given the parameters of the camera from which we wish to render an image, the point in time of the scene which we wish to render an image of, and an environment map, \oursname outputs the color of each pixel.

We start by computing the ray corresponding to that pixel and the effective specular surface from the parametric eye model.
Next we calculate the ray--specular surface intersection, retrieving the intersection location and normal vector at the intersection point. Using Snell's law, the index of refraction, the camera ray, and the normal vector, we compute the ray direction after refraction and reflection with the specular surface. This splits our original camera ray into three parts: The pre-intersect ray, the refracted ray, and the reflected ray.
We then transform equidistantly sampled points on the three rays back to our canonical volume as follows.
For each sample point on the refracted ray, we apply the inverse of the rigid transform applied to the original parametric surface.
For each sample point of the pre-intersect and reflected rays, we evaluate the warp field neural network and warp the points correspondingly.
Next, we calculate the contribution of the lighting from the environment map.
For the reflected ray, we query the environment map for the amount of incoming light from that direction.% (Note that this applies to the straight, non-warped ray)
For each sample point on all rays, we query the NeRF neural network for spherical harmonics coefficients defining a function which determines the amount of light transported from the environment map from any given angle, to the queried volume point and in the queried camera ray direction. Then, we integrate the spherical harmonics function obtained at each point over the entire environment map. %This can be greatly accelerated using a precomputation step, resulting in only needing to compute a dot product for each sample point.
Lastly, we compute the contribution of each ray towards the final result, and accumulate the radiance in each sample and from the environment map according to opacity. This produces the final RGB pixel value.

In the following, we first describe our capture setup and data (Section~\ref{sec:data}) and then explain our \oursname method in detail (Section~\ref{sec:method}). 

